Adaptation Algorithms for Neural Network-Based Speech Recognition: An Overview

We present a structured overview of adaptation algorithms for neural network-based speech recognition, considering both hybrid hidden Markov model / neural network systems and end-to-end neural network systems, with a focus on speaker adaptation, domain adaptation, and accent adaptation. The overview characterizes adaptation algorithms as based on embeddings, model parameter adaptation, or data augmentation. We present a meta-analysis of the performance of speech recognition adaptation algorithms, based on relative error rate reductions as reported in the literature.

==> eLRPD.tex <==
\begin{figure}

\centering
% Listing 1: Tex for neural network layers
\tikzsetnextfilename{eLRPD.pdf}
\begin{tikzpicture}[x=0.5cm, y=0.5cm, >=stealth]
    \tikzstyle{neuron}=[circle, draw=black, minimum size = 3mm, thick]
	
	% H1
	\draw [thick] (3.5,0) rectangle (10.5,1);
	\foreach \x in {1,...,3}
		\draw node at (3 + \x*1,0.5) [neuron] (h1_\x) {};
	\foreach \x in {1,...,3}
		\draw node at (11 - \x*1,0.5) [neuron] (h1_n-\x) {};
	\foreach \x in {1,...,3}
		\fill (7.0 -0.625 + \x*0.3,0.5) circle (1pt);
	
	% Bottleneck layer
	\draw [thick] (5,3) rectangle (9,4);
	\foreach \x in {1,...,4}
		\draw node at (4.5 + \x*1, 3.5) [neuron] (b1_\x) {};

	% Bottleneck layer
	\draw [thick] (5,6) rectangle (9,7);
	\foreach \x in {1,...,4}
		\draw node at (4.5 + \x*1, 6.5) [neuron] (b2_\x) {};

	% H2
	\draw [thick] (3.5,9) rectangle (10.5, 10);
	\foreach \x in {1,...,3}
		\draw node at (3 + \x*1, 9.5) [neuron] (h2_\x) {};
	\foreach \x in {1,...,3}
		\draw node at (11 - \x*1, 9.5) [neuron] (h2_n-\x) {};
	\foreach \x in {1,...,3}
		\fill (7.0 -0.625 + \x*0.3, 9.5) circle (1pt);

    
    % h1 -> b1
    \foreach \i in {1,...,3}
        \foreach \j in {1,...,4}
		    \draw [->,thick] (h1_\i) to (b1_\j);
	\foreach \i in {1,...,3}
        \foreach \j in {1,...,4}
		    \draw [->,thick] (h1_n-\i) to (b1_\j);
		    
    % h1 -> b1
    \foreach \i in {1,...,4}
        \foreach \j in {1,...,4}
	        \draw [->,thick] (b1_\i) to (b2_\j);
    
    % b2 -> h2   
    \foreach \i in {1,...,3}
        \foreach \j in {1,...,4}
		    \draw [->,thick] (b2_\j) to (h2_\i);
	\foreach \i in {1,...,3}
        \foreach \j in {1,...,4}
		    \draw [->,thick] (b2_\j) to (h2_n-\i);
		    
    % h1 -> h2
    \foreach \i in {1,...,3}
        \draw [->,thick, bend left=75,looseness=1.3] (h1_\i) to (h2_\i);
        \foreach \i in {1,...,3}
        \draw [->,thick, bend right=75,looseness=1.3] (h1_n-\i) to (h2_n-\i);

    \draw [thick,fill=white] (5,1.5) rectangle (9,2.5);
    \draw node at (7,2) (U) {$P \in \mathbb{R}^{n \times k}$};
    \draw [thick,fill=white] (5,4.5) rectangle (9,5.5);
    \draw node at (7,5) (E) {$T_s \in \mathbb{R}^{k \times k}$};
    \draw [thick,fill=white] (5,7.5) rectangle (9,8.5);
    \draw node at (7,8) (V) {$Q \in \mathbb{R}^{k \times n}$};
    \draw [thick,fill=white] (-0.5,4.5) rectangle (3.5,5.5);
    \draw node at (1.5,5) (D_S) {$D_s \in \mathbb{R}^{n \times n}$};

\end{tikzpicture}

\caption{A diagram of the Extended Low-Rank Plus Diagonal (eLRPD) adaptation that factorizes the adaptation matrix $A_s$ as $D_s + P T_s Q$. \ONDREJ{Should I merge figures 5,6 and 7 into one figure? It could contain diagrams for LHN, LHUC, LRPD and eLRPD}}
\label{diag:eLRPD}

\end{figure}

==> tikz/readme.tex <==
Directory required for tikz externalize.
